MTS: Bringing Multi-Tenancy to Virtual Networking

Multi-tenant cloud computing provides great benefits in terms of resource sharing, elastic pricing, and scalability, however, it also changes the security landscape and introduces the need for strong isolation between the tenants, also inside the network. This paper is motivated by the observation that while multi-tenancy is widely used in cloud computing, the virtual switch designs currently used for network virtualization lack sufficient support for tenant isolation. Hence, we present, implement, and evaluate a virtual switch architecture, MTS, which brings secure design best-practice to the context of multi-tenant virtual networking: compartmentalization of virtual switches, least-privilege execution, complete mediation of all network communication, and reducing the trusted computing base shared between tenants. We build MTS from commodity components, providing an incrementally deployable and inexpensive upgrade path to cloud operators. Our extensive experiments, extending to both micro-benchmarks and cloud applications, show that, depending on the way it is deployed, MTS may produce 1.5-2x the throughput compared to state-of-the-art, with similar or better latency and modest resource overhead (1 extra CPU). MTS is available as open source software.

==> tables/cves.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\caption{CVEs for popular virtual switches.}
\label{tab:vswitchCVEs}
%\resizebox{\textwidth}{!}{%
\scriptsize
\begin{tabular}{@{}p{2.0cm}p{4.5cm}c@{}}
%\begin{tabular}{@{}p{2.0cm}p{2.5cm}p{0.2cm}p{2.0cm}@{}}
\toprule
\textbf{Virtual Switch} & \textbf{CVEs}                                                                             & \textbf{Total} \\ \midrule
Hyper-V virtual Switch  & CVE-2017-0051, CVE-2017-0162, CVE-2017-0163, CVE-2017-0168, CVE-2017-0180, CVE-2017-0181, CVE-2017-0182, CVE-2017-0183, CVE-2017-0185 and CVE-2017-0186 & 10\\ \midrule
Nexus 1000v             & CVE-2012-0352, CVE-2013-1178, CVE-2013-1212, CVE-2013-1213, CVE-2013-3400, CVE-2013-5556 and CVE-2015-0775                     & 7\\ \midrule
Open vSwitch            & CVE-2012-3449, CVE-2016-2074, CVE-2016-10377, CVE-2017-9214, CVE-2017-9263, CVE-2017-9264, CVE-2017-9265 and CVE-2017-14970 & 8\\ \midrule
VMware vSwitch          & None                                                                                      & 0\\ \bottomrule
\end{tabular}%
%}
\end{table}


==> tables/extended-baseline-tput.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\normalsize
\caption{Throughput for the Baseline mode with more compute and memory resources.}
\label{tab:extended-baseline-tput}
%\scriptsize
\centering
\begin{tabular}{@{}p{4.0cm}p{0.4cm}p{0.4cm}p{0.4cm}@{}}
\toprule
 & \multicolumn{3}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Throughput (Mpps)\\ in Traffic Scenario\end{tabular}}} \\ \cmidrule(l){2-4}
\textbf{Vswitch Mode} & \textbf{p2p} & \textbf{p2v} & \textbf{v2v} \\ \midrule
Baseline 2 Cores & 1.5 & 0.2 & 0.1 \\
Baseline 4 Cores & 3.0 & 0.2 & 0.1 \\
Baseline Dpdk 2 Cores & 14.0 & 5.6 & 3.5 \\
Baseline Dpdk 4 Cores & 14.0 & 7.9 & 5.5 \\ \bottomrule
\end{tabular}
\end{table}


==> tables/resources.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\normalsize
\caption{Resource allocation for security levels. \gabor{kash: please, describe correctly in the figure caption what is that we see in the table (how many tenants we are assuming, etc.) and please also add the number of VFs required in each case. Also, please make the table more compact, it takes too much space right now.}}
\label{tab:resources}
\scriptsize
\centering

\begin{tabular}{@{}p{2.0cm}p{1.0cm}p{1.0cm}p{1.0cm}@{}}
\toprule
\multicolumn{1}{l}{\textbf{Resource Allocation Strategy}} & \multicolumn{1}{l}{\textbf{Security Level}}               & \multicolumn{1}{l}{\textbf{CPU}} & \multicolumn{1}{l}{\textbf{Memory}} \\ \midrule
\multirow{4}{*}{Shared}                                   & Baseline                                                  & 1                                & 1                                   \\ \cmidrule(l){2-4}
                                                          & Level 1                                                   & 1                                & 2                                   \\ \cmidrule(l){2-4}
                                                          & \multirow{2}{*}{Level 2}                                  & 2                                & 3                                   \\ \cmidrule(l){3-4}
                                                          &                                                           & 4                                & 5                                   \\ \midrule
\multirow{8}{*}{Isolated}                                 & Baseline                                                  & 1                                & 1                                   \\ \cmidrule(l){2-4}
                                                          & Level 1                                                   & 1                                & 2                                   \\ \cmidrule(l){2-4}
                                                          & \multirow{2}{*}{Level 2}                                  & 2                                & 3                                   \\ \cmidrule(l){3-4}
                                                          &                                                           & 4                                & 5                                   \\ \cmidrule(l){2-4}
                                                          & \begin{tabular}[c]{@{}c@{}}Baseline +\\ Dpdk\end{tabular} & 2                                & 1.25                                \\ \cmidrule(l){2-4}
                                                          & \multirow{3}{*}{Level 3}                                  & 1                                & 2                                   \\ \cmidrule(l){3-4}
                                                          &                                                           & 2                                & 3                                   \\ \cmidrule(l){3-4}
                                                          &                                                           & 4                                & 4                                   \\ \bottomrule
\end{tabular}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

